Reproducibility in NLP: What Have We Learned from the Checklist?

Scientific progress in NLP rests on the reproducibility of researchers' claims. The *CL conferences created the NLP Reproducibility Checklist in 2020 to be completed by authors at submission to remind them of key information to include. We provide the first analysis of the Checklist by examining 10,405 anonymous responses to it. First, we find evidence of an increase in reporting of information on efficiency, validation performance, summary statistics, and hyperparameters after the Checklist's introduction. Further, we show acceptance rate grows for submissions with more Yes responses. We find that the 44% of submissions that gather new data are 5% less likely to be accepted than those that did not; the average reviewer-rated reproducibility of these submissions is also 2% lower relative to the rest. We find that only 46% of submissions claim to open-source their code, though submissions that do have 8% higher reproducibility score relative to those that do not, the most for any item. We discuss what can be inferred about the state of reproducibility in NLP, and provide a set of recommendations for future conferences, including: a) allowing submitting code and appendices one week after the deadline, and b) measuring dataset reproducibility by a checklist of data collection practices.

==> abstract_old.tex <==
\begin{abstract}
% Like all sciences, Natural Language Processing (NLP) faces the challenge of producing results that can be reproduced. 
Scientific progress in NLP relies on our claims being robust and reproducible.
The *CL conferences created the NLP Reproducibility Checklist, which is filled out at submission by authors, and is designed to remind authors of important reproducibility information they should include in their papers.
%With the aim of facing the scientific challenge of producing reproducible results, *CL conferences created the NLP Reproducibility Checklist which consists of items .
%This reminder asks authors which of a set of key details are included at submission time.
In this work, we provide the first analysis of the NLP Reproducibility Checklist by analyzing more than 10,000 (anonymous) responses to the checklist.
%We have gathered all (anonymized) submission data from the first four conferences that used the NLP reproducibility checklist: \TheConfs, totaling more than 10,000 submissions.
%To better understand the reproducibility practices used by the community, we examine the results of these checklists from \TheConfs\.
%We find that with notable exceptions, these practices are frequently reported and submissions reporting them are more often accepted and perceived as reproducible by *CL reviewers.
First, we have evidence that the introduction of the checklist led to more frequent reporting of reproducibility information, and that more \Yes\ responses to the checklist items associate with higher acceptance rates.
The checklist responses offer interesting insights into publication patterns in our field, including that 44\% of submissions created new data, but those submissions had 
a 5\%
lower acceptance rate than submissions that didn't create new data.
%We find that 44\% of 
%However, we find that the $44\%$ of submissions presenting new data are accepted less and viewed as less reproducible.
%These gaps are not attributable to non-reporting of any of the current checklist items, suggesting the need for more fine-grained measurements of data collection practices.
Additionally, we find only $46\%$ of submissions claim to open-source their code, and this has the largest impact on reviewer-percevied reproducibility of a submission out of any checklist item.
%but find that closed source submissions frequently lack reporting on efficiency measures and even evaluation metrics, which are otherwise difficult or impossible to infer without open source code.
%Additionally, we find a $46\%$ rate of open source code, which is comparable to previous studies, but find that closed source submissions frequently lack reporting on efficiency measures and even evaluation metrics, which are otherwise difficult or impossible to infer without open source code.
Lastly we find that a majority of reviewers found the checklist to be useful and even find evidence that rates of some less adopted reproducibility practices have increased since the checklist implementation.

\end{abstract}




%another version after Jesse's comments 

% Scientific progress in LP rests on the repro. ancibility of our claims. 'The sCL.conterences created the LP Reproducibility Checklist, which is completed by authors at submission to remind them of key information to include We provide the first analysis of the Checklist by examining 13.655 anonymous responses. First. we find evidence of an increase in efficiency,
% Valldacion, summary statistes, and aypeoparan eter reporting alter the Checanst's introduction
% Further, acceptance rate grows for submissions with more "Yes" responses. We find that the 41% of submissions presentine new data are
% 5% less likely to be accepted than those that
% did not Average reviewer-fated reproducibility for these is also 2% lower. We find only 46%
% of submissions claim to open-source their code. though doing so increases average reviewer rated reproducibility by 8%, the largest for any ilem. For more complete reporting we recom-mend: a conterences should allow submitling code, appendices, and checklists one week after the deadline, and b) dataset reproducibility
% shonid be measured he a checeast of date col.
